On the Significance of Consecutive Ballots in Paxos

In this paper we examine the Paxos protocol and demonstrate how the discrete numbering of ballots can be leveraged to weaken the conditions for learning. Specifically, we define the notion of consecutive ballots and use this to define Consecutive Quorums. Consecutive Quorums weakens the learning criterion such that a learner does not need matching $accept$ messages sent in the $same \; ballot$ from a majority of acceptors to learn a value. We prove that this modification preserves the original safety and liveness guarantees of Paxos. We define $Consecutive \; Paxos$ which encapsulates the properties of discrete consecutive ballots. To establish the correctness of these results, we, in addition to a paper proof, formally verify the correctness of a State Machine Replication Library built on top of an optimized version of Multi-Paxos modified to reflect $Consecutive \; Paxos$.

==> Sections/PaxosProof.tex <==
\section{Paxos Proof of Safety}\label{paxos_proof}
We begin by showing a proof of safety for Paxos, which will help clarify the proofs for both Consecutive Quorums and Consecutive Proposals.  Paxos has both $Liveness$ and $Safety$ properties. In this paper we focus only on $Safety$. The changes to the protocol do not make any changes that could affect $Liveness$.

To prove the safety of Paxos we need to show that by following the above phases, \textit{"Only a single value can be learned"}. A value could be \textit{learned} after a majority of acceptors accept the same value in the same ballot. Value $v$ is \textit{chosen} and could become learned in ballot $i$ if, $\exists Q_i : \forall r \in Q_i : 2B(i,v,r_a) \in sent_k$. This states that all acceptors in a majority quorum have sent identical $2B$ messages for value $v$ in the same ballot, $i$. Using this definition, the following is a formal description of the $Safety$ property:
\begin{theorem}[Safety Theorem]
\label{safetyTheorem}
No two different values can be learned
\[ \forall i,j \in \mathbb{Z^+} : [\exists Q_i : \forall r \in Q_i : 2B(i,v,r_a) \in sent_r 
                 \land \exists Q_j : \forall r' \in Q_j : 2B(j,w,r'_a) \in sent_{r'}] \implies v = w \]
\end{theorem}

Safety Theorem \ref{safetyTheorem} states, if value $v$ was learned in ballot $i$ and value $w$ was learned in ballot $j$, it must be the case that $v$ and $w$ are identical.

To prove that Safety Theorem \ref{safetyTheorem} holds for Paxos, we prove the following three Lemmas over all ballots $i$ and $j \in \mathbb{Z^+}$.
\begin{lemma}
\label{lemma1}[Equal]
If $v$ is chosen in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot $j == i$
\end{lemma}

\begin{lemma}
\label{lemma2}[Less Than]
If $v$ is chosen in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot  $j < i$
\end{lemma}

\begin{lemma}
\label{lemma3}[Greater Than]
If $v$ is chosen in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot  $j > i$
\end{lemma}

By showing that Lemmas \ref{lemma1}, \ref{lemma2}, and \ref{lemma3} hold, it is straight forward to prove that the safety of Paxos is ensured. The safety theorem deals with all ballots $i,j$; the above three lemmas cover all cases, when $i == j, i < j,$ and $i > j$. Therefore Lemma \ref{lemma1} $\land$ Lemma \ref{lemma2} $\land$ Lemma \ref{lemma3} $\implies$ Safety Theorem.

\iffalse
A value is considered to be \textit{learned} when there is at least a majority quorum of replicas that send a 2B message for the same value in the same ballot. Value $v$ is said to be \textit{learned} if $\exists Q :: \forall a \in Q :: 2B(i,v,a)$
 ... \fi

To help prove the above Lemmas we make use of the following definitions that are implicit with the specification of Paxos:
\theoremstyle{definition}
\begin{definition}
\label{LearnImpliesAccept}[Learn Implies Accept]
If value $v$ is Learned in ballot $i$, then $v$ must have been Accepted by at least one acceptor in ballot $i$.
\end{definition}

\begin{definition}
\label{AcceptImpliesPropose}[Accept Implies Propose]
If value $v$ is Accepted in ballot $i$ (by some acceptor), then $v$ must have been Proposed in ballot $i$.
\end{definition}

We can combine Definitions  \ref{LearnImpliesAccept},and \ref{AcceptImpliesPropose} using transitivity to define a third equivalent Definition.

\begin{definition}

\label{LearnImpliesPropose}[Learn Implies Propose]
If value $v$ is Learned in ballot $i$, then $v$ must have been Proposed in ballot $i$.
\end{definition} 

For the ease of proving Lemma \ref{lemma1}, we can further break the problem into Lemma \ref{lemma1a}. A proof of Lemma \ref{lemma1a} along with the definition \textit{Learn Implies Accept} (\ref{LearnImpliesAccept}), proves, using Transitivity Lemma \ref{lemma1}. 
\begin{customlemma}{3.1'}
\label{lemma1a}
If an acceptor has accepted $v$ in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot $j == i$
\end{customlemma}

\iffalse
A proof of Lemma \ref{lemma1a} along with the definition \textit{Learn Implies Accept} (\ref{LearnImpliesAccept}), proves, using Transitivity Lemma \ref{lemma1}. 

By using definition \textit{Learn Implies Accept} (\ref{LearnImpliesAccept}) and showing that Lemma \ref{lemma1a} is true, with Transitivity, Lemma \ref{lemma1} also holds. 

Note how the consequent of Definition \ref{LearnImpliesAccept} matches the antecedent of Lemma \ref{lemma1a}. If Lemma \ref{lemma1a} is true, using transitivity we have proven the following: \textit{If value $v$ is learned in ballot $i$, then no other value $w \neq v$ could be chosen in any ballot $j == i$. }

\fi 


\begin{proof}
To prove Lemma \ref{lemma1a}, we know that $i == j$, and at least one acceptor has accepted value $v$ in ballot $i$. There must be at least one acceptor that has accepted $v$ in ballot $j$. From Definition \textit{Accept Implies Propose} (\ref{AcceptImpliesPropose}), we know that $v$ was proposed in ballot $j$. To finish this proof, we can rely on the construction of Paxos itself. Only a single unique value can be proposed per ballot. $v$ was already proposed in ballot $i$, so no other value could be proposed. A value can not be learned if it was not proposed.  No $w \neq v$ could possibly be learned in ballot $j == i$.
\end{proof}

\iffalse
\noindent Similarly, we can approach Lemma \ref{lemma2} and Lemma \ref{lemma3} as follows:
\begin{customlemma}{3.2'}
\label{lemma2a}
If an acceptor has accepted $v$ in ballot $i$ then no other value $w \neq v$  could be chosen in any ballot $j < i$
\end{customlemma}
By using \textit{Learn Implies Accept} (\ref{LearnImpliesAccept}) and showing that Lemma \ref{lemma2a} is true, with Transitivity, Lemma \ref{lemma2} also holds. 

\begin{customlemma}{3.3'}
\label{lemma3a}
If $v$ is chosen in ballot $i$, then no value $w \neq v$  could be proposed in any ballot $j > i$
\end{customlemma}

Lemma \ref{lemma3a} is structured slightly different than the previous lemmas. Using the contrapositive of \textit{Learn Implies Propose} (\ref{LearnImpliesPropose}) and showing that Lemma \ref{lemma3a} is true, Lemma \ref{lemma3} is proven with Transitivity.

On inspection, it appears as if Lemma \ref{lemma2} and Lemma \ref{lemma3} are symmetrical. In order to take advantage of this, we show that Lemma \ref{lemma3a} $\implies$ Lemma \ref{lemma2a}. This is done by taking the contrapositive of Lemma \ref{lemma2a}, and using Definition \textit{Accept Implies Propose} (\ref{AcceptImpliesPropose}).  Lemma \ref{lemma3a} shows that if any value is learned in \textbf{any} ballot $i$ then no other value could be proposed in any higher ballot. The result of transforming Lemma \ref{lemma2a} states that if a value was learned in a \textbf{single} ballot, then no other value could be proposed in any higher ballot. This follows that by proving Lemma \ref{lemma3a}, we can also directly show that Lemma \ref{lemma2a} holds. By proving these two Lemmas, both Lemma \ref{lemma3} and Lemma \ref{lemma2} can be be shown directly. To prove Lemma \ref{lemma2} and Lemma \ref{lemma3}, it is sufficient to just prove Lemma \ref{lemma3a}. See Appendix \ref{apendix:a} for a more detailed explanation.
\fi

To prove the Safety Theorem for all ballots $i,j \in \mathbb{Z^+}$, there can be two cases, $i == j$ or $i \neq j$. If $i \neq j$, it is either the case that $i < j$ (Lemma \ref{lemma3}) or $i > j$ (Lemma \ref{lemma2}). We can rely on the symmetrical nature of this relationship and focus on proving Lemma \ref{lemma3}. The proof for Lemma \ref{lemma2} can be derived from the proof for Lemma \ref{lemma3}. See Appendix \ref{apendix:a} for a more detailed explanation and expanded proof.

Similarly to the proof for Lemma \ref{lemma1}, we can first define and prove Lemma \ref{lemma3a}. Using the contrapositive of \textit{Learn Implies Propose} (\ref{LearnImpliesPropose}) and showing that Lemma \ref{lemma3a} is true, Lemma \ref{lemma3} is proven with Transitivity.

\begin{customlemma}{3.3'}
\label{lemma3a}
If $v$ is chosen in ballot $i$, then no value $w \neq v$  could be proposed in any ballot $j > i$
\end{customlemma}

\begin{proof} To prove Lemma \ref{lemma3a} we use an inductive argument on $r \geq 1$ for all ballots $b \geq i+r$. 

\textbf{Base Case:} $r == 1$. The proposer in ballot $i+1$ must obtain a $Q$ of valid $1B$ messages before proposing a value. From quorum intersection, there must be at least one acceptor that sends a $1B$ message to the proposer in ballot $i+1$ that also sent a $2B$ message for $v$ in ballot $i$. This overlapping acceptor will contain the highest $maxVB$ in the quorum. There are no ballots higher than $i$ that could be reported in ballot $i+1$, proposer $p$ will propose the same value $v$. 

\textbf{Inductive Step:} Assume that no proposer in the span of ballots $i ... i+r-1$ proposed a value $w \neq v$. We show that the proposer in ballot $i+r$ will also not propose  $w \neq v$. 

The proposer in ballot  $i+r$ must obtain a $Q$ of valid $1B$ messages before proposing a value. From quorum intersection, there must be at least one acceptor that sends a $1B$ message to the proposer in ballot $i+r$ that also sent a $2B$ message in some ballot $\geq i$. The highest reported $maxVB$ will be at least as large as $i$. From the inductive hypothesis, the only value that was proposed and could have been accepted in this span is $v$. The proposer in ballot $i+r$ must propose $v$.
\end{proof}

From this result, we have shown that Lemmas \ref{lemma1}, \ref{lemma2}, and \ref{lemma3} hold, and prove the safety of Paxos.

The additional information carried by Consecutive Ballots in Paxos is used as part of the above proof. The inductive proof for the safety of Paxos relies on the fact that given two consecutive ballots, $i$ and $i+1$, there can be no intermediary ballot that is higher than $i$, but still less than $i+1$. A replica observing these consecutive ballots gains the certainty that there exist no intermediary ballots that could contain any contradictory information. The information in consecutive ballots can be used to help prove the safety of Paxos and can be extended to safely weaken both the criteria to learn a value and the criteria for a proposer to propose.

==> Sections/s5_ConsecutiveP.tex <==
\section{Consecutive Proposals} \label{consecPSection}

% Fix this first sentence *
% Quorums in Paxos are used both to learn and propose values, leveraging consecutive ballots, the criteria for proposing values can be weakened. 

We now introduce "Consecutive Proposals", showing how to use consecutive ballots to weaken the criteria for proposing values. For ease of explanation, we present Consecutive Proposals without considering Consecutive Quorums. In Classic Paxos, a proposer must obtain $promise$ messages from a majority of acceptors before knowing what values are safe to propose. In contrast, a Consecutive Proposal allows a proposer to propose a value immediately after receiving a $promise$ message from the consecutive previous ballot. 

We can define the criteria for a proposer $\pi$ to propose a value in Classic Paxos with the following definition. Proposer $\pi$ can create and send a valid $propose$ message in ballot $i$ when the listed criteria is met. 
\begin{definition}
\label{PaxosPropose}[Normal Proposal]

% \[2A(i,v,p) \equiv \exists Q_i : 
%     [(\forall \alpha \in Q_i : \promise{\perp}{\perp} \in msgs_p  \land \alpha.maxVB = \; \perp) 
%              \]
%     \[ \qquad \lor (\exists \alpha \in Q_i : 1B(i,j,v,\alpha)\in msgs_p \;\] \[\qquad \qquad \qquad \qquad \land \;(\forall \gamma \in Q_i : 1B(i,j',w,\gamma)\in msgs_p \land j \geq j' ) ]\]



\[ \exists \propose{i}{v}{\pi} \iff \exists Q_i .\; 
[(\forall \alpha \in Q_i .\; \promise{i}{\bot}{\alpha} \in msgs_\pi)\] 
\[ \qquad \qquad \qquad \qquad \qquad \qquad 
    \lor \; ((\exists \alpha \in Q_i .\; \promise{i}{\proposal{j}{v}}{\alpha} \in msgs_\pi) \] 
\[ \qquad \qquad \qquad \qquad \qquad \qquad  \qquad \qquad \qquad \qquad
    \land \; (\forall \gamma \in Q_i .\; \promise{i}{\proposal{j'}{w}}{\gamma} \in msgs_\pi \land j \geq j')) ]  \]

\end{definition}


If a proposer obtains a quorum of $promise$ messages in ballot $i$, and one of the $promise$ messages received is from an acceptor that accepted $v$ in the previous ballot $i-1$, the proposer will propose $v$. It does not matter what other proposals the other received $promise$ messages contain; regardless, the ballot from $i-1$ will be the highest possible reported ballot. Ballots $i$ and $i-1$ are consecutive.
A proposer waiting for a majority of $promise$ messages can safely propose a value before receiving a full quorum, as long as the proposer has received at least one $promise$ message from the consecutive previous ballot.

We define the criteria for proposer $\pi$ to immediately create and send a $propose$ message in ballot $i$ using consecutive ballots as a Consecutive Proposal. 
\begin{definition}
\label{consecP}[Consecutive Proposal]

% \[2A(i,v,p) \equiv \exists \alpha :  1B(i,i-1,v,\alpha) \in msgs_p\]
\[ \exists\propose{i}{v}{\pi} \iff \exists \alpha .\; \promise{i}{\proposal{i-1}{v}}{\alpha} \in msgs_\pi\]
\end{definition}

% With these two definitions detailing the criteria to propose a value, we can further define when a proposer is eligible to propose a value using either a Normal Proposal or a Consecutive Proposal;

% %This still feels awkward.. 
% \begin{align*}
%     Normal \; Proposal \equiv Definition \ref{PaxosPropose}\\
%     Consecutive \; Proposal \equiv \; ! Definition \ref{PaxosPropose} \land Definition \ref{consecP}
% \end{align*}
A proposer will immediately send a $propose$ message when either the criteria for a Normal Proposal, or a Consecutive Proposal is met. In the case that a proposer waiting for a quorum of $promise$ messages, has received $f$ responses (one less than required for a full quorum of $f+1$), and the final response is a Consecutive promise, the proposal will be treated as a Normal Proposal. This demonstrates the case where both the Consecutive Proposal and Normal Proposal criteria are satisfied at the same time. The action and value proposed will be the same in both cases, but a Normal Proposal has the additional property that a majority of acceptors have promised to not participate in any previous ballot.

% A Consecutive Proposal will only take place when the criteria for a Normal Proposal is not met, and the proposer has received the appropriate consecutive promise message. If the size of the quorum of promise messages acquired by the proposer is $f$ and the final promise message arrives, the proposer will proceed with a Normal Proposal regardless if the last promise message was consecutive. 
% The action and value proposed will be the same in both cases, but some implicit side effects cause the two to differ.

As observed in Fast Paxos\cite{FastPaxos} for reconfiguration, an $accept$ message contains the same information as a $promise$ message from the same acceptor. This can be used to extend the definition of a Consecutive Proposal. A $promise$ $message$ contains the proposal that the source acceptor has most recently accepted a value in. With our model, an agent can operate as multiple roles and could receive both $promise$ and $accept$ messages. This model of an agent operating as multiple roles is standard in practical settings\cite{Ironfleet,PaxosLive,libpaxos,Spanner}. Otherwise, an acceptor could broadcast the $accept$ message to all agents rather then just to the learners. An $accept$ message sent to agent $\theta$ from an acceptor for value $v$ in ballot $i-1$ will contain the identical information sent by that same acceptor to agent $\theta$ in a $promise$ message in ballot $i$. We can use this to further extend the definition of a Consecutive Proposal to be valid if the proposer observes a $promise$ message from an acceptor that accepted a value in the previous ballot or an $accept$ message from an acceptor in the previous ballot. For proposer $\pi$, this is formally defined as:
\begin{definition}
\label{consecP_wAccept}[Consecutive Proposal Extended] 
% \[2A(i,v,p) \equiv \exists \alpha :  1B(i,i-1,v,\alpha) \in msgs_p
%         \lor 2B(i-1,v,\alpha) \in msgs_p \]
    
\[ \exists\propose{i}{v}{\pi} \iff \exists \alpha .\; \promise{i}{\proposal{i-1}{v}}{\alpha} \in msgs_\pi 
\lor \accept{i-1}{v}{\alpha} \in msgs_\pi\]

\end{definition}

Relinquishing the necessity for quorums seems to directly contradict the foundation of safety that Paxos relies on. By having a proposer potentially propose a value after only hearing back from a single acceptor, could lead to a string of proposals only supported by a stream of single acceptors. Consecutive Proposals do not extract a promise that a majority of acceptors will not participate in a previous ballot. Regardless, this does not compromise safety. To help explain why, we define and prove the following two corollaries. 

\begin{corollary}[Normal Before Consecutive]
\label{consecPNormalFirst}
There must exist at least one \textbf{Normal Proposal} before any Consecutive Proposals can take place.
\end{corollary}

\begin{proof}
We prove Corollary \ref{consecPNormalFirst} by contradiction, assume a Consecutive Proposal happens before any Normal Proposal. For a Consecutive Proposal to take place, the proposer must receive either a non-null $promise$ message or an $accept$ message from the consecutive previous ballot. Recursively all previous proposals were Consecutive Proposals, which implies that the first possible proposal was Consecutive. The first proposal can not have been based on any valid non-null $promise$ or $accept$ messages from an earlier ballot. A Consecutive Proposal can not propose a new value. This is a contradiction, at least one Normal Proposal must have occurred before any Consecutive Proposal. 
\end{proof}

\begin{corollary}[Consecutive Same Value]
\label{consecPConsecSameVal}
A Consecutive Proposal can only propose the same value that was proposed in the most recent Normal Proposal.
\end{corollary}

\begin{proof}
We prove Corollary \ref{consecPConsecSameVal} by contradiction, assume that a Consecutive Proposal contains a different value than the most recent Normal Proposal. For a Consecutive Proposal to occur, a replica must have observed either a $promise$ or an $accept$ message from the consecutive previous ballot. We must consider two cases, that the proposal in the consecutive previous ballot was either a Normal Proposal or a Consecutive Proposal.
\begin{enumerate}
    \item \textbf{Normal Proposal:} Only a single value can be proposed per ballot. The value in the observed $promise$ or $accept$ message must contain the value that was proposed in the previous ballot. Based on the definition of Consecutive Proposals, the proposer will propose this same value, which is a contradiction. 
    \item \textbf{Consecutive Proposal:} Based on the definition of Consecutive Proposals, the proposer will propose the same value that was proposed in this ballot. Inductively this pattern will repeat until the previous $promise$ or $accept$ message was based on a Normal Proposal. A chain of Consecutive Proposals will all propose the same value. This eventually leads to a contradiction from the Normal Proposal case. 
\end{enumerate}

\end{proof}

The above two corollaries help form an informal argument to the safety of Consecutive Proposals. A Consecutive Proposal relies on receiving an $accept$ message or a non-null $promise$ message, neither can exist before an initial value is proposed in a Normal Proposal. A Consecutive Proposal does not rely on a full quorum but is either preceded immediately by a Normal Proposal, and will propose the same value, or will be preceded by another Consecutive Proposal. Inductively, this Consecutive Proposal will propose the same value as the most recent Normal Proposal.

An acceptor sending a $promise$ message to a new proposer serves two purposes. First, the acceptor relays the highest numbered proposal it has previously accepted \proposal{n'}{v'}, if any, to the proposer. Secondly, this acceptor promises to not participate in any ballots less than the current ballot started by the new proposer. Without Consecutive Proposals, every successful quorum of $promise$ messages implies that there is a majority of acceptors that will not participate in any previous ballots. Consecutive Proposals do not maintain this, it is possible for a value to be proposed based on a proposer receiving a single message. Even though a majority of acceptors could participate in an earlier ballot, safety is still preserved. 

Consider an execution of Paxos using Consecutive Proposals where ballot number $k > 0$ is the first instance of a Consecutive Proposal. From Corollary \ref{consecPNormalFirst} (\textit{Normal Before Consecutive}), and the definition of Consecutive Proposals, the proposal in ballot $k-1$ must have been a Normal Proposal. The Normal Proposal in ballot $k-1$ was made based on a majority quorum of $promise$ messages. The first $k-1$ ballots are no different than Classic Paxos, so safety is preserved in this span. From the definition of Consecutive Proposals, the proposer in ballot $k$ must propose the same value that was proposed in the Normal Proposal from ballot $k-1$. Following ballot $k$ there could be a series of $i$ additional ballots that have Consecutive Proposals. This series of $i$ Consecutive Proposals do not have a full quorum of $promise$ messages. From the construction of a Consecutive Proposal, each Consecutive Proposal in the span of $k$ to $k+i$ can only propose the same value as the previous ballot. From Corollary \ref{consecPConsecSameVal} (\textit{Consecutive Same Value}), this value is the same as the value proposed in the most recent Normal Proposal from ballot $k-1$. Even though these proposals do not have a majority quorum of promises to not participate in a previous ballot, there was a majority that promised in ballot $k-1$. Even if there is a late arriving message for a different value, it must have come from a proposal prior to  ballot $k-1$. At least a majority of acceptors will ignore it based on the promise in ballot $k-1$. Since a majority of acceptors will ignore any previous messages, a different value can not be chosen in this span. There will never exist a majority of acceptors that accept a different value in this interim. The first ballot after the span of Consecutive Proposals is a Normal Proposal, ballot $k+i+1$. The proposer in ballot $k+i+1$ will obtain a majority quorum of $promise$ messages, and choose to propose the value associated with the highest reported ballot. If a value has already been chosen, from quorum intersection there will be at least one acceptor in common. If the value was chosen before ballot $k-1$, then all proposals in between must have contained the same value. If the value was learned on or after ballot $k-1$, the series of Consecutive Proposals only propose this same value. This covers the case that the reported proposal from this overlapping acceptor is not the largest, no different value could have been proposed in a higher ballot. If no value has previously been chosen then no matter what value is proposed, there now exists a full quorum of acceptors who promise to ignore any messages from previous ballots, preventing a different previous value becoming chosen. This prevents a potentially different value becoming learned as the result of some belated Consecutive Proposal. After this pattern of Normal-Consecutive-Normal is complete, there again exists a majority of acceptors who promise to not participate in a previous ballot less than $k+i+1$.


% The proposer in ballot $k+i+1$ will obtain a majority quorum of promise messages, and choose to propose the value associated with the highest reported ballot. This highest ballot will either fall in the span of $k$ to $k+i$, or will be the same highest ballot observed in the Normal Proposal from ballot $k-1$. Either way, the same value will be proposed. After this pattern of Normal-Consecutive-Normal is complete, there again exists a majority of acceptors who promise to not participate in a previous ballot less than $k+i+1$.
%FIX ^^ DOESN'T QUITE MAKE SENSE! -- I think it is OK now..  


Even without the promise of a majority of other acceptors to not participate in previous ballots, Consecutive Proposals preserve safety. From Corollary \ref{consecPConsecSameVal} (\textit{Consecutive Same Value}), Consecutive Proposals are limited to propose the same value as the most recent Normal Proposal. Based on a majority of acceptors promising to not participate in an earlier ballot from the most recent Normal Proposal, A majority quorum can not form that chooses a different value. An additional difference between Consecutive Proposals and Normal Proposals is that Consecutive Proposals do not guarantee that there can be only one value proposed per ballot. Normal Proposals ensure that only a single value can be proposed per ballot because a majority of acceptors need to respond to a proposer's $prepare$ message before any proposer can propose a value. There will never be two distinct majority quorums that form in a single ballot allowing multiple proposers to propose a value. With Consecutive Proposals, multiple values can be proposed in the same ballot. However, all values proposed in the same ballot will have the same value. If multiple proposers attempt to propose values for the same ballot, the acceptors will receive one proposal before the other and will ignore any other proposals for that ballot. This behavior is the same as in Classic Paxos, an acceptor will ignore duplicate or extra messages for the same ballot. These proposals carry the same value from the same ballot, there is no harm in these additional proposals. By having a distinguished proposer and a method for electing new leaders, dueling proposals can be avoided.

\subsection{Safety Proof For Consecutive Proposals}

The proof of safety for the addition of Consecutive Proposals mirrors the proof for Consecutive Quorums, the lemmas we prove are the same, but the proof differs. The Safety Property \ref{safetyTheorem} and the definitions remain the same. The difference, however, is how proposers can safely propose values. For the sake of presenting Consecutive Quorums and Consecutive Proposals separately, for this proof the criteria for choosing values is the same as in Classic Paxos, Definition \ref{chosenDef}. We define and prove the following Lemmas:

\iffalse
To prove the safety of Consecutive Proposals, we modify the safety proof for Classic Paxos. The safety property stated in \ref{safetyTheorem} is still the same, the difference is how proposers can safely propose values. To prove the safety property, adapting the same strategy as before, we define Lemmas \ref{lemma1P}, \ref{lemma2P}, and \ref{lemma3P} show correctness. The proof for both \ref{lemma1P}, and \ref{lemma2P} is the same as for Classic Paxos. This is the proof for \ref{lemma3P}. To prove \ref{lemma3P}, we prove \ref{lemma3Pa} and through transitivity obtain \ref{lemma3P}.
\fi

\begin{lemma}
\label{lemma1P}[Equal Consecutive Proposals]
If $v$ is chosen in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot $j = i$
\end{lemma}

\begin{lemma}
\label{lemma2P}[Less Than Consecutive Proposals]
If $v$ is chosen in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot  $j < i$
\end{lemma}

\begin{lemma}
\label{lemma3P}[Greater Than Consecutive Proposals]
If $v$ is chosen in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot  $j > i$
\end{lemma}

We prove Lemma \ref{lemma1P} by first proving Lemma \ref{lemma1Pa} and then applying transitivity to obtain our result for Lemma \ref{lemma1P}. Similarly to prove Lemma \ref{lemma3P}, we first prove Lemma \ref{lemma3Pa} and then apply transitivity to obtain our result for Lemma \ref{lemma2P} and Lemma \ref{lemma3P}. The proof for Lemma \ref{lemma2P} also follows directly from \ref{lemma3P}. 

\begin{customlemma}{5.1'}
\label{lemma1Pa}
If an acceptor has accepted $v$ in ballot $i$ then no other value $w \neq v$ could be chosen in any ballot $j = i$
\end{customlemma}

\begin{proof}
To prove Lemma \ref{lemma1Pa}, we know that $i = j$, and at least one acceptor has accepted $v$ in ballot $i$. There must be at least one acceptor that has accepted $v$ in ballot $j$. From Definition \textit{Accept Implies Propose} (\ref{AcceptImpliesPropose}), we know that $v$ was proposed in ballot $j$. If $v$ was proposed as a Normal Proposal, then we can assert that $v$ was the only value proposed in ballot $j$. If the proposal in ballot $j$ was a Consecutive Proposal, it is possible that it was not the only proposal. However, if there was more than one Consecutive Proposal then all values proposed were the same. $v$ was already proposed in ballot $i$. Only $v$ can be proposed in ballot $j$. A value can not be chosen if it was not proposed. No $w \neq v$ could possibly be chosen in ballot $j = i$.
\end{proof}

\begin{customlemma}{5.3'}
\label{lemma3Pa}
If $v$ is chosen in ballot $i$, then no value $w \neq v$  could be proposed in any ballot $j > i$
\end{customlemma}

\begin{proof}We prove Lemma \ref{lemma3Pa} by induction on $r \geq 1$ for all ballots $j \geq i+r$, but must distinguish between Normal Proposals and Consecutive Proposals.  Assume that value $v$ \textit{has been chosen in ballot $i$}, and call the majority quorum of acceptors that chose this value $Q_i$.

\noindent \textbf{Base Case:} $r = 1$. Suppose some proposer proposed a value in ballot $j = i+1$. The proposal in ballot $j=i+1$ can be either a Normal or Consecutive Proposal. 

\begin{enumerate}
    \item \textbf{Normal Proposal}: This is the same as in Classic Paxos. The proposer in ballot $i+1$ must obtain a quorum of valid $promise$ messages before proposing a value. From quorum intersection, there must be at least one acceptor that sends a $promise$ message to the proposer in ballot $i+1$ that is also in $Q_i$. This overlapping acceptor will contain the highest proposal in the quorum. There are no ballots higher than $i$ that could be reported in ballot $i+1$, proposer $p$ will propose the same value $v$. 
    
    \item \textbf{Consecutive Proposal}: In order for the proposal in ballot $i+1$ to be Consecutive, the proposer must have received either an $accept$ message or a $promise$ message from an acceptor in $Q_i$. From the definition of a Consecutive Proposal, the proposer must propose $v$.
\end{enumerate}
  
\noindent \textbf{Inductive Step:} Assume that no proposer in the span of ballots $i, \dots, i+r-1$ proposed a value $w \neq v$. We show that the proposer in ballot $i+r$ will also not propose  $w \neq v$. Again, we must consider the case that the proposal in ballot $i+r$ is either a Normal Proposal or a Consecutive Proposal. 
\begin{enumerate}
    \item \textbf{Normal Proposal}: There could have been Consecutive Proposals in the span from $i$ to $i+r-1$. The proposer in ballot  $i+r$ must obtain a quorum of valid $promise$ messages before proposing a value. From quorum intersection, there must be at least one acceptor that sent a $promise$ message to the proposer in ballot $i+r$ that also is in $Q_i$. The highest reported proposal will be no smaller than $i$. From the inductive hypothesis, only $v$ can be proposed between ballot $i$ and the $i+r-1$. If there was a span of Consecutive Proposals in the range $i + 1$ to $i+r$, the inductive hypothesis ensures that the same value will be proposed. Without extracting promises, these intermediary acceptors may accept a previous different value. This previous different value must have been from a ballot $< i$, and cannot be the highest proposal reported to the proposer in ballot $i+r$. No majority of acceptors that all accept a different value $w \neq v$ could form. $v$ remains the only value that is eligible to propose.
    
    \item \textbf{Consecutive Proposal}: For the proposal in ballot $i+r$ to be a Consecutive Proposal, there must have been a value proposed in ballot $i+r-1$. From the inductive hypothesis, the proposer in ballot $i+r-1$ must have proposed $v$. By the definition of a Consecutive Proposal, the proposer in ballot $i$ must have received either an $accept$ message from ballot $i+r-1$, or a $promise$ message for ballot $i+r$ from an acceptor that accepted $v$ in ballot $i+r-1$. The proposer must propose $v$.
\end{enumerate}
\end{proof}

From this result, we have proved Lemmas \ref{lemma1P}, \ref{lemma2P}, and \ref{lemma3P}, and thus prove the safety of Paxos with Consecutive Proposals.

% To formally verify that the addition of Consecutive Quorums does not violate Paxos's safety property, we modified the verified version of SMR based on multi-Paxos from the IronFleet project. We modified the protocol specification to include Consecutive Quorums and showed a refinement to the high-level specification of the SMR library. 

% In a practical setting, to implement Consecutive Quorums as described above would require that each replica has access to unlimited memory. Due to the asynchronous environment, a replica would need to keep track of all messages from previous ballots that could potentially be used to form a Consecutive Quorum. Messages may take arbitrarily long to arrive, a replica may need to keep track of unlimited messages from previous ballots. 

% To overcome this issue, we implemented Consecutive Quorums in a manner that is slightly less 'weak', but still weaker than in Classic Paxos. To do so, we maintained a consecutive set of messages from increasing numbered ballots, only adding new messages if their addition to the set did not break the consecutive definition. This is less weak than the version described above but is still safe because even in Classic Paxos is it is valid for a Replica to ignore a message and still preserve correctness. This also still fulfils the definition of Consecutive Quorums, but does not keep track of all possible messages. By only keeping track of a running Consecutive Quorum of ballots, the refinement proof was straightforward to show. This is because the criteria that a quorum had a cardinality of $|f+1|$ is still sufficient to learn a value, based on the construction of the quorum. It was still vital to make sure that each incoming ballot being added to the consecutive quorum had matching values and was for the same slot in multi-Paxos. 

% A key lemma to show this result was to prove that once a valid quorum of 2B messages formed, either Normal or Consecutive, any future 2A message must have the matching value. We were able to show this using quorum intersection and that from the definitions of both types of quorums, all values in the quorums must have the same value. 

% \subsection{Formal Verification of Consecutive Proposals}
% The approach to formally verify Consecutive Proposals paralleled the process for Consecutive Quorums. Starting with the correctly proved version of SMR based on multi-Paxos from IronFleet, we modified the protocol specification to include the definition of Consecutive Proposals. Similar to our system model, IronFleet allows replicas to act as multiple roles. We modified a replica to internally send a specially crafted 1B message to itself upon receiving the correct consecutive 2B message, so a proposer only internally deals with 1B messages. The information remains equivalent between the 1B and 2B message, so the change preserves the Consecutive Proposal
% definition.

% We needed to prove the same key lemma as with Consecutive Quorums, once a valid 2B quorum forms to learn a value, any future 2A messages must contain the same value. This similarly mirrors Lemma \ref{lemma3Pa}. To prove this, we were not able to rely on quorum intersection in all cases. The proof changed depending on the type of proposal that formed the 2A message. The proof for a Normal Proposal remained the same as the original case. If the 2A message was the result of a Consecutive Proposal, we were able to reason about the consecutive 1B message that satisfied the definition of the Consecutive Proposal, either the original 1B message or the crafted 1B based on the consecutive 2B message. Using a recursive proof, we were able to show that given a 2A message proposed by a Consecutive Proposal, that all 2A consecutive messages between the 2B quorum and the current 2A message had the same value. 

\subsection{Phase-1 Bypass}
In the case that a process acts as multiple agents and can receive all types of messages, using Consecutive Proposals, a view change could happen and bypass Phase 1 of Paxos. A new proposer can successfully propose a value $v$ in ballot $i$ if the proposer receives a valid $promise$ or $accept$ message from the previous ballot ($i-1$). An agent may receive an $accept$ message for value $v$ in ballot $i-1$, and then immediately suspect that the current proposer has crashed. Depending on the election procedure, if this agent is elected as the distinguished proposer, it may proceed immediately with proposing a value. This agent already has the correct criteria to propose a value in ballot $i$ and can do so bypassing the first whole half of Paxos. 

==> TLA/TLA_ConsecP.tex <==
\tlatex
\setboolean{shading}{true}
\@x{}\moduleLeftDash\@xx{ {\MODULE} Consecutive Proposals}\moduleRightDash\@xx{}%
\@pvspace{8.0pt}%
\@x{ {\EXTENDS} Integers ,\, Naturals ,\, TLC}%
\@x{}
\@pvspace{8.0pt}%
\@x{ {\CONSTANT} Value ,\, Acceptor ,\, Quorum}%
\@pvspace{8.0pt}%
 \@x{ {\ASSUME} QuorumAssumption \.{\defeq} \.{\land} \A\, Q \.{\in} Quorum
 \.{:} Q \.{\subseteq} Acceptor}%
 \@x{\@s{145.19} \.{\land} \A\, Q1 ,\, Q2 \.{\in} Quorum \.{:} Q1 \.{\cap} Q2
 \.{\neq} \{ \}}%
\@pvspace{8.0pt}%
\@x{ Ballot \.{\defeq}\@s{4.1} Int}%
\@pvspace{8.0pt}%
\@x{ None \.{\defeq} {\CHOOSE} v \.{:} v \.{\notin} Ballot}%
\@pvspace{16.0pt}%
 \@x{ Message \.{\defeq}\@s{20.5} [ type\@s{2.83} \.{:} \{\@w{1a} \} ,\,
 bal\@s{1.93} \.{:} Ballot ]}%
 \@x{\@s{49.10} \.{\cup}\@s{15.97} [ type\@s{2.83} \.{:} \{\@w{1b} \} ,\, acc
 \.{:} Acceptor ,\, bal \.{:} Ballot ,\,}%
 \@x{\@s{78.97} mbal \.{:} Ballot \.{\cup} \{ \.{-} 1 \} ,\, mval \.{:} Value
 \.{\cup} \{ None \} ]}%
 \@x{\@s{49.10} \.{\cup}\@s{15.97} [ type\@s{2.83} \.{:} \{\@w{2a} \} ,\,
 bal\@s{1.93} \.{:} Ballot ,\, val \.{:} Value ]}%
 \@x{\@s{49.10} \.{\cup}\@s{15.97} [ type\@s{2.83} \.{:} \{\@w{2b} \} ,\, acc
 \.{:} Acceptor ,\, bal \.{:} Ballot ,\, val \.{:} Value ]}%
\@x{}
\@x{ {\VARIABLE} maxBal ,\,}%
\@x{\@s{46.84} maxVBal ,\,}%
\@x{\@s{46.84} maxVal ,\,}%
\@x{\@s{46.84} msgs}%
\@pvspace{24.0pt}%
 \@x{ vars \.{\defeq} {\langle} maxBal ,\, maxVBal ,\, maxVal ,\, msgs
 {\rangle}}%
\@pvspace{8.0pt}%
 \@x{ TypeOK \.{\defeq} \.{\land} maxBal \.{\in} [ Acceptor \.{\rightarrow}
 Ballot \.{\cup} \{ \.{-} 1 \} ]}%
 \@x{\@s{56.14} \.{\land} maxVBal \.{\in} [ Acceptor \.{\rightarrow} Ballot
 \.{\cup} \{ \.{-} 1 \} ]}%
 \@x{\@s{56.14} \.{\land} maxVal \.{\in} [ Acceptor \.{\rightarrow} Value
 \.{\cup} \{ None \} ]}%
\@x{\@s{56.14} \.{\land} msgs \.{\subseteq} Message}%
\@pvspace{16.0pt}%
 \@x{ Init \.{\defeq} \.{\land} maxBal \.{=} [ a \.{\in} Acceptor \.{\mapsto}
 \.{-} 1 ]}%
 \@x{\@s{35.70} \.{\land} maxVBal \.{=} [ a \.{\in} Acceptor \.{\mapsto} \.{-}
 1 ]}%
 \@x{\@s{35.70} \.{\land} maxVal \.{=} [ a \.{\in} Acceptor \.{\mapsto} None
 ]}%
\@x{\@s{35.70} \.{\land} msgs \.{=} \{ \}}%
\@pvspace{16.0pt}%
\@x{ Send ( m ) \.{\defeq} msgs \.{'} \.{=} msgs \.{\cup} \{ m \}}%
\@pvspace{16.0pt}%
 \@x{ Phase1a ( b ) \.{\defeq} \.{\land} Send ( [ type \.{\mapsto}\@w{1a} ,\,
 bal \.{\mapsto} b ] )}%
 \@x{\@s{69.22} \.{\land} {\UNCHANGED} {\langle} maxBal ,\, maxVBal ,\, maxVal
 {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Phase1b ( a ) \.{\defeq} \.{\land} \E\, m \.{\in} msgs \.{:}}%
\@x{\@s{84.43} \.{\land} m . type \.{=}\@w{1a}}%
\@x{\@s{84.43} \.{\land} m . bal \.{>} maxBal [ a ]}%
 \@x{\@s{84.43} \.{\land} maxBal \.{'} \.{=} [ maxBal {\EXCEPT} {\bang} [ a ]
 \.{=} m . bal ]}%
 \@x{\@s{84.43} \.{\land} Send ( [ type \.{\mapsto}\@w{1b} ,\, acc \.{\mapsto}
 a ,\, bal \.{\mapsto} m . bal ,\,}%
 \@x{\@s{128.29} mbal \.{\mapsto} maxVBal [ a ] ,\, mval \.{\mapsto} maxVal [
 a ] ] )}%
\@x{\@s{69.22} \.{\land} {\UNCHANGED} {\langle} maxVBal ,\, maxVal {\rangle}}%
\@pvspace{16.0pt}%
\@x{ Clause1 ( b ,\, v ) \.{\defeq} \E\, Q \.{\in} Quorum \.{:}}%
 \@x{\@s{89.63} \.{\LET} Q1b \.{\defeq} \{ m \.{\in} msgs\@s{6.20} \.{:}
 \.{\land} m . type \.{=}\@w{1b}}%
\@x{\@s{211.35} \.{\land} m . acc \.{\in} Q}%
\@x{\@s{211.35} \.{\land} m . bal\@s{1.57} \.{=} b \}}%
 \@x{\@s{114.13} Q1bv \.{\defeq} \{ m \.{\in} Q1b \.{:} m . mbal \.{\geq} 0
 \}}%
 \@x{\@s{89.63} \.{\IN}\@s{4.09} \.{\land} \A\, a \.{\in} Q \.{:} \E\, m
 \.{\in} Q1b \.{:} m . acc \.{=} a}%
\@x{\@s{114.13} \.{\land} \.{\lor} Q1bv \.{=} \{ \}}%
\@x{\@s{129.34} \.{\lor} \E\, m \.{\in} Q1bv \.{:}}%
\@x{\@s{144.55} \.{\land} m . mval \.{=} v}%
 \@x{\@s{144.55} \.{\land} \A\, mm \.{\in} Q1bv \.{:} m . mbal \.{\geq} mm .
 mbal}%
\@pvspace{16.0pt}%
 \@x{ Clause2 ( b ,\, v ) \.{\defeq}\@s{4.1} \E\, m \.{\in} msgs \.{:}
 \.{\lor} \.{\land} m . type\@s{3.34} \.{=}\@w{1b}}%
\@x{\@s{153.13} \.{\land} m . mbal\@s{0.51} \.{=} b \.{-} 1}%
\@x{\@s{153.13} \.{\land} m . mval \.{=} v}%
\@x{\@s{153.13} \.{\land} m . bal \.{=} b}%
\@x{\@s{142.02} \.{\lor} \.{\land} m . type \.{=}\@w{2b}}%
\@x{\@s{153.13} \.{\land} m . bal\@s{0.51} \.{=} b \.{-} 1}%
\@x{\@s{153.13} \.{\land} m . val \.{=} v}%
\@pvspace{24.0pt}%
\@x{ NormalProposal ( b ,\, v ) \.{\defeq} Clause1 ( b ,\, v )}%
\@pvspace{8.0pt}%
 \@x{ ConsecProposal ( b ,\, v )\@s{1.93} \.{\defeq} {\lnot} Clause1 ( b ,\, v
 ) \.{\land}\@s{4.1} Clause2 ( b ,\, v )}%
\@pvspace{8.0pt}%
\@x{ Phase2a ( b ,\, v ) \.{\defeq}}%
 \@x{\@s{8.2} \.{\land} {\lnot} \E\, m \.{\in} msgs \.{:} m . type
 \.{=}\@w{2a} \.{\land} m . bal \.{=} b}%
 \@x{\@s{8.2} \.{\land} ( NormalProposal ( b ,\, v ) \.{\lor} ConsecProposal (
 b ,\, v ) )}%
 \@x{\@s{8.2} \.{\land} Send ( [ type \.{\mapsto}\@w{2a} ,\, bal \.{\mapsto} b
 ,\, val \.{\mapsto} v ] )}%
 \@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} maxBal ,\, maxVBal ,\, maxVal
 {\rangle}}%
\@pvspace{24.0pt}%
 \@x{ Phase2b ( a ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land} m . type
 \.{=}\@w{2a}}%
\@x{\@s{128.83} \.{\land} m . bal \.{\geq} maxBal [ a ]}%
 \@x{\@s{128.83} \.{\land} maxBal \.{'} \.{=} [ maxBal {\EXCEPT} {\bang} [ a ]
 \.{=} m . bal ]}%
 \@x{\@s{128.83} \.{\land} maxVBal \.{'} \.{=} [ maxVBal {\EXCEPT} {\bang} [ a
 ] \.{=} m . bal ]}%
 \@x{\@s{128.83} \.{\land} maxVal \.{'} \.{=} [ maxVal {\EXCEPT} {\bang} [ a ]
 \.{=} m . val ]}%
 \@x{\@s{128.83} \.{\land} Send ( [ type \.{\mapsto}\@w{2b} ,\, acc
 \.{\mapsto} a ,\,}%
 \@x{\@s{168.59} bal \.{\mapsto} m . bal ,\, val\@s{2.06} \.{\mapsto} m . val
 ] )}%
\@pvspace{8.0pt}%
 \@x{ Next \.{\defeq} \.{\lor} \E\, b\@s{0.64} \.{\in} Ballot \.{:} \.{\lor}
 Phase1a ( b )}%
\@x{\@s{112.86} \.{\lor} \E\, v \.{\in} Value \.{:} Phase2a ( b ,\, v )}%
 \@x{\@s{39.83} \.{\lor} \E\, a \.{\in} Acceptor \.{:} Phase1b ( a ) \.{\lor}
 Phase2b ( a )}%
\@pvspace{8.0pt}%
\@x{ Spec\@s{1.46} \.{\defeq} Init \.{\land} {\Box} [ Next ]_{ vars}}%
\@pvspace{16.0pt}%
 \@x{ Sent2b ( a ,\, v ,\, b ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land}
 m . type \.{=}\@w{2b}}%
\@x{\@s{145.63} \.{\land} m . acc \.{=} a}%
\@x{\@s{145.63} \.{\land} m . val\@s{1.06} \.{=} v}%
\@x{\@s{145.63} \.{\land} m . bal\@s{1.57} \.{=} b}%
\@pvspace{8.0pt}%
 \@x{ Sent2a ( v ,\, b ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land} m .
 type \.{=}\@w{2a}}%
\@x{\@s{134.28} \.{\land} m . val \.{=} v}%
\@x{\@s{134.28} \.{\land} m . bal\@s{0.51} \.{=} b}%
\@pvspace{16.0pt}%
 \@x{ NormalBeforeSpec ( b ,\, v ) \.{\defeq} \.{\land} ConsecProposal ( b ,\,
 v )}%
\@x{\@s{123.88} \.{\land} \E\, x \.{\in} Ballot \.{:} \.{\land} x \.{<} b}%
\@x{\@s{196.88} \.{\land} NormalProposal ( x ,\, v )}%
\@pvspace{8.0pt}%
 \@x{ SpecSameValAsLastNorm ( b ,\, v ) \.{\defeq} \.{\land} ConsecProposal (
 b ,\, v )}%
\@x{\@s{155.95} \.{\land} \E\, x \.{\in} Ballot \.{:} \.{\land} x \.{<} b}%
\@x{\@s{228.94} \.{\land} NormalProposal ( x ,\, v )}%
 \@x{\@s{228.94} \.{\land} \A\, y \.{\in} Ballot \.{:} ( y \.{>} x \.{\land} y
 \.{\leq} b ) \.{\implies} ConsecProposal ( y ,\, v )}%
\@pvspace{16.0pt}%
 \@x{ Agreed ( v ,\, b ) \.{\defeq} \E\, Q \.{\in} Quorum \.{:} \A\, a \.{\in}
 Q \.{:} Sent2b ( a ,\, v ,\, b )}%
\@pvspace{16.0pt}%
 \@x{ NoFutureProposal ( v ,\, b ) \.{\defeq} \A\, v2 \.{\in} Value \.{:} \A\,
 b2 \.{\in} Ballot \.{:} ( b2 \.{>} b \.{\land} Sent2a ( v2 ,\, b2 ) )
 \.{\implies} v \.{=} v2}%
\@pvspace{8.0pt}%
 \@x{ SafeValue \.{\defeq} \A\, v \.{\in} Value \.{:} \A\, b \.{\in} Ballot
 \.{:} Agreed ( v ,\, b ) \.{\implies} NoFutureProposal ( v ,\, b )}%
\@pvspace{8.0pt}%
 \@x{ SpecSafety \.{\defeq} \A\, v \.{\in} Value \.{:} \A\, b \.{\in} Ballot
 \.{:} ConsecProposal ( b ,\, v ) \.{\implies} NormalBeforeSpec ( b ,\, v )
 \.{\land} SpecSameValAsLastNorm ( b ,\, v )}%
\@pvspace{8.0pt}%
\@x{}\bottombar\@xx{}%

==> TLA/TLA_ConsecQ.tex <==
\tlatex
\setboolean{shading}{true}
\@x{}\moduleLeftDash\@xx{ {\MODULE} Consecutive Quorums}\moduleRightDash\@xx{}%
\@x{ {\EXTENDS} Integers ,\, Naturals ,\, TLC}%
\@x{ {\CONSTANT} Value ,\, Acceptor ,\, Quorum}%
\@pvspace{8.0pt}%
 \@x{ {\ASSUME} QuorumAssumption \.{\defeq} \.{\land} \A\, Q \.{\in} Quorum
 \.{:} Q \.{\subseteq} Acceptor}%
 \@x{\@s{145.19} \.{\land} \A\, Q1 ,\, Q2 \.{\in} Quorum \.{:} Q1 \.{\cap} Q2
 \.{\neq} \{ \}}%
\@pvspace{8.0pt}%
\@x{ Ballot \.{\defeq}\@s{4.1} Int}%
\@pvspace{8.0pt}%
\@x{ None \.{\defeq} {\CHOOSE} v \.{:} v \.{\notin} Ballot}%
\@pvspace{8.0pt}%
 \@x{ PrintVal ( id ,\, exp )\@s{4.1} \.{\defeq}\@s{4.1} Print ( {\langle} id
 ,\, exp {\rangle} ,\, {\TRUE} )}%
\@pvspace{8.0pt}%
 \@x{ Message \.{\defeq}\@s{20.5} [ type\@s{2.83} \.{:} \{\@w{1a} \} ,\,
 bal\@s{1.93} \.{:} Ballot ]}%
 \@x{\@s{49.10} \.{\cup}\@s{15.97} [ type\@s{2.83} \.{:} \{\@w{1b} \} ,\, acc
 \.{:} Acceptor ,\, bal \.{:} Ballot ,\,}%
 \@x{\@s{78.97} mbal \.{:} Ballot \.{\cup} \{ \.{-} 1 \} ,\, mval \.{:} Value
 \.{\cup} \{ None \} ]}%
 \@x{\@s{49.10} \.{\cup}\@s{15.97} [ type\@s{2.83} \.{:} \{\@w{2a} \} ,\,
 bal\@s{1.93} \.{:} Ballot ,\, val \.{:} Value ]}%
 \@x{\@s{49.10} \.{\cup}\@s{15.97} [ type\@s{2.83} \.{:} \{\@w{2b} \} ,\, acc
 \.{:} Acceptor ,\, bal \.{:} Ballot ,\, val \.{:} Value ]}%
\@pvspace{8.0pt}%
\@x{ {\VARIABLE} maxBal ,\,}%
\@x{\@s{46.84} maxVBal ,\,}%
\@x{\@s{46.84} maxVal ,\,}%
\@x{\@s{46.84} msgs}%
\@pvspace{8.0pt}%
 \@x{ vars \.{\defeq} {\langle} maxBal ,\, maxVBal ,\, maxVal ,\, msgs
 {\rangle}}%
\@x{ Send ( m ) \.{\defeq} msgs \.{'} \.{=} msgs \.{\cup} \{ m \}}%
\@pvspace{8.0pt}%
 \@x{ TypeOK \.{\defeq} \.{\land} maxBal \.{\in} [ Acceptor \.{\rightarrow}
 Ballot \.{\cup} \{ \.{-} 1 \} ]}%
 \@x{\@s{56.14} \.{\land} maxVBal \.{\in} [ Acceptor \.{\rightarrow} Ballot
 \.{\cup} \{ \.{-} 1 \} ]}%
 \@x{\@s{56.14} \.{\land} maxVal \.{\in} [ Acceptor \.{\rightarrow} Value
 \.{\cup} \{ None \} ]}%
\@x{\@s{56.14} \.{\land} msgs \.{\subseteq} Message}%
\@pvspace{8.0pt}%
 \@x{ Init \.{\defeq} \.{\land} maxBal \.{=} [ a \.{\in} Acceptor \.{\mapsto}
 \.{-} 1 ]}%
 \@x{\@s{35.70} \.{\land} maxVBal \.{=} [ a \.{\in} Acceptor \.{\mapsto} \.{-}
 1 ]}%
 \@x{\@s{35.70} \.{\land} maxVal \.{=} [ a \.{\in} Acceptor \.{\mapsto} None
 ]}%
\@x{\@s{35.70} \.{\land} msgs \.{=} \{ \}}%
\@pvspace{8.0pt}%
 \@x{ Phase1a ( b ) \.{\defeq} \.{\land} Send ( [ type \.{\mapsto}\@w{1a} ,\,
 bal \.{\mapsto} b ] )}%
 \@x{\@s{69.22} \.{\land} {\UNCHANGED} {\langle} maxBal ,\, maxVBal ,\, maxVal
 {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Phase1b ( a ) \.{\defeq} \.{\land} \E\, m \.{\in} msgs \.{:}}%
\@x{\@s{84.43} \.{\land} m . type \.{=}\@w{1a}}%
\@x{\@s{84.43} \.{\land} m . bal \.{>} maxBal [ a ]}%
 \@x{\@s{84.43} \.{\land} maxBal \.{'} \.{=} [ maxBal {\EXCEPT} {\bang} [ a ]
 \.{=} m . bal ]}%
 \@x{\@s{84.43} \.{\land} Send ( [ type \.{\mapsto}\@w{1b} ,\, acc \.{\mapsto}
 a ,\, bal \.{\mapsto} m . bal ,\,}%
 \@x{\@s{128.29} mbal \.{\mapsto} maxVBal [ a ] ,\, mval \.{\mapsto} maxVal [
 a ] ] )}%
\@x{\@s{69.22} \.{\land} {\UNCHANGED} {\langle} maxVBal ,\, maxVal {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Phase2a ( b ,\, v ) \.{\defeq}}%
 \@x{\@s{8.2} \.{\land} {\lnot} \E\, m \.{\in} msgs\@s{7.89} \.{:} m . type
 \.{=}\@w{2a} \.{\land} m . bal \.{=} b}%
\@x{\@s{8.2} \.{\land} \E\, Q \.{\in} Quorum \.{:}}%
 \@x{\@s{26.53} \.{\LET} Q1b \.{\defeq} \{ m \.{\in} msgs\@s{6.20} \.{:}
 \.{\land} m . type \.{=}\@w{1b}}%
\@x{\@s{148.25} \.{\land} m . acc \.{\in} Q}%
\@x{\@s{148.25} \.{\land} m . bal\@s{1.57} \.{=} b \}}%
\@x{\@s{51.03} Q1bv \.{\defeq} \{ m \.{\in} Q1b \.{:} m . mbal \.{\geq} 0 \}}%
 \@x{\@s{26.53} \.{\IN}\@s{4.09} \.{\land} \A\, a \.{\in} Q \.{:} \E\, m
 \.{\in} Q1b \.{:} m . acc \.{=} a}%
\@x{\@s{51.03} \.{\land} \.{\lor} Q1bv \.{=} \{ \}}%
\@x{\@s{62.14} \.{\lor} \E\, m\@s{7.71} \.{\in} Q1bv \.{:}}%
\@x{\@s{81.45} \.{\land} m . mval \.{=} v}%
 \@x{\@s{81.45} \.{\land} \A\, mm \.{\in} Q1bv \.{:} m . mbal \.{\geq} mm .
 mbal}%
 \@x{\@s{8.2} \.{\land} Send ( [ type \.{\mapsto}\@w{2a} ,\, bal \.{\mapsto} b
 ,\, val \.{\mapsto} v ] )}%
 \@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} maxBal ,\, maxVBal ,\, maxVal
 {\rangle}}%
\@pvspace{8.0pt}%
 \@x{ Phase2b ( a ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land} m . type
 \.{=}\@w{2a}}%
\@x{\@s{128.83} \.{\land} m . bal \.{\geq} maxBal [ a ]}%
 \@x{\@s{128.83} \.{\land} maxBal \.{'} \.{=} [ maxBal {\EXCEPT} {\bang} [ a ]
 \.{=} m . bal ]}%
 \@x{\@s{128.83} \.{\land} maxVBal \.{'} \.{=} [ maxVBal {\EXCEPT} {\bang} [ a
 ] \.{=} m . bal ]}%
 \@x{\@s{128.83} \.{\land} maxVal \.{'} \.{=} [ maxVal {\EXCEPT} {\bang} [ a ]
 \.{=} m . val ]}%
 \@x{\@s{128.83} \.{\land} Send ( [ type \.{\mapsto}\@w{2b} ,\, acc
 \.{\mapsto} a ,\,}%
 \@x{\@s{168.59} bal \.{\mapsto} m . bal ,\, val\@s{2.06} \.{\mapsto} m . val
 ] )}%
\@pvspace{8.0pt}%
 \@x{ Next \.{\defeq} \.{\lor} \E\, b\@s{0.64} \.{\in} Ballot \.{:} \.{\lor}
 Phase1a ( b )}%
\@x{\@s{112.86} \.{\lor} \E\, v \.{\in} Value \.{:} Phase2a ( b ,\, v )}%
 \@x{\@s{39.83} \.{\lor} \E\, a \.{\in} Acceptor \.{:} Phase1b ( a ) \.{\lor}
 Phase2b ( a )}%
\@pvspace{8.0pt}%
\@x{ Spec\@s{1.46} \.{\defeq} Init \.{\land} {\Box} [ Next ]_{ vars}}%
\@pvspace{8.0pt}%
\@x{ NotIn ( Q ,\, a ) \.{\defeq} a \.{\notin} Q}%
\@pvspace{8.0pt}%
 \@x{ ConsecQ ( Q ,\, b ,\, v ) \.{\defeq}\@s{4.1} \A\, r \.{\in} Acceptor
 \.{:} NotIn ( Q ,\, r ) \.{\land} \E\, m\@s{10.13} \.{\in} msgs \.{:}
 \.{\land} m . type \.{=}\@w{2b}}%
\@x{\@s{228.60} \.{\land} m . acc \.{=} r}%
 \@x{\@s{228.60} \.{\implies} \.{\lor} ( \A\, q \.{\in} Q \.{:} \E\, n \.{\in}
 msgs \.{:} \.{\land} n . type \.{=}\@w{2b}}%
\@x{\@s{359.19} \.{\land} n . acc\@s{5.42} \.{=} q}%
\@x{\@s{359.19} \.{\implies} m . bal \.{<} n . bal )}%
 \@x{\@s{244.16} \.{\lor} ( \A\, q \.{\in} Q \.{:} \E\, n \.{\in} msgs \.{:}
 \.{\land} n . type \.{=}\@w{2b}}%
\@x{\@s{359.19} \.{\land} n . acc\@s{2.86} \.{=} q}%
\@x{\@s{359.19} \.{\implies} n . bal \.{<} m . bal )}%
\@pvspace{8.0pt}%
 \@x{ Sent2b ( a ,\, v ,\, b ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land}
 m . type \.{=}\@w{2b}}%
\@x{\@s{145.63} \.{\land} m . acc \.{=} a}%
\@x{\@s{145.63} \.{\land} m . val\@s{1.06} \.{=} v}%
\@x{\@s{145.63} \.{\land} m . bal\@s{1.57} \.{=} b}%
\@pvspace{8.0pt}%
 \@x{ Sent2bNoBal ( a ,\, v ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land} m
 . type \.{=}\@w{2b}}%
\@x{\@s{161.94} \.{\land} m . acc \.{=} a}%
\@x{\@s{161.94} \.{\land} m . val\@s{1.06} \.{=} v}%
\@pvspace{8.0pt}%
 \@x{ Sent2a ( v ,\, b ) \.{\defeq} \E\, m \.{\in} msgs \.{:} \.{\land} m .
 type \.{=}\@w{2a}}%
\@x{\@s{134.28} \.{\land} m . val \.{=} v}%
\@x{\@s{134.28} \.{\land} m . bal\@s{0.51} \.{=} b}%
\@pvspace{8.0pt}%
 \@x{ AgreedConsecQ ( v ,\, b ) \.{\defeq} \E\, Q \.{\in} Quorum \.{:}\@s{4.1}
 \.{\land} \A\, a \.{\in} Q \.{:} Sent2bNoBal ( a ,\, v )}%
\@x{\@s{189.74} \.{\land} \E\, a \.{\in} Q \.{:} Sent2b ( a ,\, v ,\, b )}%
\@x{\@s{189.74} \.{\land} ConsecQ ( Q ,\, b ,\, v )}%
\@pvspace{16.0pt}%
 \@x{ Agreed ( v ,\, b ) \.{\defeq} \E\, Q \.{\in} Quorum \.{:} \A\, a \.{\in}
 Q \.{:} Sent2b ( a ,\, v ,\, b )}%
 \@x{ NoFutureProposal ( v ,\, b ) \.{\defeq} \A\, v2 \.{\in} Value \.{:} \A\,
 b2 \.{\in} Ballot \.{:} ( b2 \.{>} b \.{\land} Sent2a ( v2 ,\, b2 ) )
 \.{\implies} v \.{=} v2}%
\@pvspace{8.0pt}%
 \@x{ SafeValue \.{\defeq} \A\, v \.{\in} Value \.{:} \A\, b \.{\in} Ballot
 \.{:} AgreedConsecQ ( v ,\, b )\@s{4.1} \.{\implies} NoFutureProposal ( v
 ,\, b )}%
\@pvspace{8.0pt}%
\@x{}\bottombar\@xx{}%
